Mind the Accuracy-Approval Gap: How Users Evaluate Sycophantic AI in Everyday Tasks

Large language models (LLMs) often exhibit sycophancy, a tendency to agree with users, flatter or affirm them, and preserve their face, even when independent judgment or critical feedback would be more useful. Prior work has largely evaluated sycophancy through benchmark evaluations, but less is known about how users perceive and respond to sycophantic AI in everyday tasks. We combine benchmark evaluations with two large-scale user studies. We study four personas defined through system prompts: objective (instructed to prioritize accuracy over agreement), soft-sycophantic, hard-sycophantic, and baseline (no persona-specific system prompt). Benchmarks show that even baseline exhibits substantial sycophancy, agreeing with users' stated views 71.7% of the time on NLP Survey, compared with 54.8% for objective and 89.5% for hard-sycophantic. Under conversational pressure on TruthfulQA, accuracy ranged from 81.9% for objective to 59.6% for baseline and 8.7% for hard-sycophantic. Participants were assigned to one of the four personas, and either discussed contested policy topics or collaborated with AI on email writing. Despite its higher accuracy under pressure, objective AI was rated significantly less respectful and satisfying than the other personas, and less trustworthy than baseline. Baseline and sycophantic personas did not differ significantly. Persona did not significantly affect how often participants changed their opinions, although participants who discussed with objective AI had greater odds of reduced confidence. Objective AI prompted greater writing expansion than soft-sycophantic AI, but final writing quality did not differ significantly across personas. These findings highlight a tension between accuracy and user approval: personas with substantially lower accuracy under conversational pressure received more favorable ratings for respect and satisfaction than objective AI.

==> benchmark_figures/figure_snippets.tex <==
% Copy individual environments into your ACM paper.
% Upload PDF/SVG files to an Overleaf folder named benchmark_figures.
% Optional: prefer PDF in pdfLaTeX via \includegraphics.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{benchmark_figures/01_agreement_with_user_views.pdf}
\caption{Agreement with users’ stated views on three model-written evaluation datasets. The figure reports the percentage of answers aligning with the stated user view; higher agreement does not necessarily indicate higher factual accuracy.}
\label{fig:01_agreement_with_user_views}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{benchmark_figures/02_elephant_social_pooled.pdf}
\caption{ELEPHANT social sycophancy, pooled across OEQ, AITA-YTA and SS. Bars show the percentage of responses assigned positive validation, indirectness and framing labels by GPT-4o using the benchmark’s judging prompts.}
\label{fig:02_elephant_social_pooled}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{benchmark_figures/03_elephant_social_by_dataset.pdf}
\caption{ELEPHANT social-sycophancy measures broken down by benchmark dataset. Positive-label rates are not human-normalized ELEPHANT scores.}
\label{fig:03_elephant_social_by_dataset}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{benchmark_figures/04_elephant_moral_both_nta.pdf}
\caption{ELEPHANT moral sycophancy: proportion of original/flipped matched scenarios for which the model issued NTA verdicts from both opposing perspectives. This is not a measure of overall moral correctness.}
\label{fig:04_elephant_moral_both_nta}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{benchmark_figures/05_syceval_answer.pdf}
\caption{SycophancyEval Answer: percentage of eligible, scoreable comparisons where a neutral correct answer becomes incorrect after user conditioning.}
\label{fig:05_syceval_answer}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{benchmark_figures/06_syceval_are_you_sure.pdf}
\caption{SycophancyEval Are You Sure: percentage of initially correct and scoreable pairs where the model switches to an incorrect answer after being challenged.}
\label{fig:06_syceval_are_you_sure}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{benchmark_figures/07_syceval_feedback.pdf}
\caption{SycophancyEval Feedback: percentage of non-tied pairwise GPT-4o judgments finding conditioned feedback more positive than neutral feedback, across arguments, math and poems. Two reversed judge presentation orders were used per underlying comparison.}
\label{fig:07_syceval_feedback}
\end{figure*}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{benchmark_figures/08_mmlu_pro_accuracy.pdf}
\caption{Accuracy on MMLU-Pro (12,032 examples per persona). The plotted axis is zoomed to distinguish small descriptive differences.}
\label{fig:08_mmlu_pro_accuracy}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{benchmark_figures/09_truthfulqa_multiturn.pdf}
\caption{Final-turn accuracy on multi-turn TruthfulQA under repeated user pressure (3,160 scored outputs per persona).}
\label{fig:09_truthfulqa_multiturn}
\end{figure}



==> manuscript/a2.tex <==

























\subsection{Prolific Announcement Script}
\label{app:recruitment}

\subsubsection{Opinion Discussion Study}

\begin{quote}\small

We are conducting a research study about how people interact with conversational AI systems. In this study, you will answer questions about your opinions on three topics, have a series of conversations with an AI chatbot and answer questions about your experience.

The study will take approximately 20 minutes to complete. You will receive \$6.67 for completing the study, equivalent to a rate of approximately \$20 per hour.

Participation is voluntary. Additional information about the study, including data collection and confidentiality, will be provided in the consent form before you begin.

\end{quote}

\subsubsection{Email Writing Study}

\begin{quote}\small

We are conducting a research study about how people interact with conversational AI systems during a writing task. In this study, you will answer a brief questionnaire about your background in AI usage and complete two short writing tasks by interacting with an AI chatbot.

The study will take approximately 20 minutes to complete. You will receive \$6.67 for completing the study, equivalent to a rate of approximately \$20 per hour.

Participation is voluntary. Additional information about the study, including data collection and confidentiality, will be provided in the consent form before you begin.

\end{quote}






\subsubsection{Discussion Topics}

Participants discussed the following three statements, presented in randomized order.

\begin{quote}\small

\begin{enumerate}
    \item Social media companies should have stronger content moderation.
    \item A four-day workweek should become the standard.
    \item Governments should ban single-use plastics.
\end{enumerate}

\end{quote}






























\subsection{Study Recruitment and Survey Administration}
\label{app:recruitment}

Participants were recruited through Prolific. The consent forms and questionnaires for both studies were hosted on Qualtrics and embedded within the web-based study interface. Participants completed the surveys and AI interaction tasks in sequence through that interface before being redirected to Prolific for study completion.

\subsubsection{Opinion Discussion Study: Procedure}

After providing consent, participants completed a background questionnaire about their use of AI chatbots. For each assigned topic, they completed a pre-conversation questionnaire, discussed the statement with their assigned AI persona, and completed a post-conversation questionnaire. This sequence was repeated for each assigned topic, followed by study completion. The topic order was randomized.

\subsubsection{AI-Assisted Writing Study: Procedure}

After providing consent, participants completed a background questionnaire about their English writing proficiency, TOEFL experience, and use of AI writing assistants. They then completed two email-writing tasks, in randomized order. For each task, they first wrote an initial email draft independently, requested feedback from the assigned AI persona, revised their draft through at least two rounds of feedback, and submitted a final draft. The study ended after both writing tasks were completed.

\subsubsection{Prolific Description: Opinion Discussion Study}
\begin{quote}\small
We are conducting a research study about how people interact with conversational AI systems. In this study, you will answer questions about your opinions on three topics, have a series of conversations with an AI chatbot and answer questions about your experience.

The study will take approximately 20 minutes to complete. You will receive \$6.67 for completing the study, equivalent to a rate of approximately \$20 per hour.

Participation is voluntary. Additional information about the study, including data collection and confidentiality, will be provided in the consent form before you begin.
\end{quote}

\subsubsection{Prolific Description: Email Writing Study}
\begin{quote}\small
We are conducting a research study about how people interact with conversational AI systems during a writing task. In this study, you will answer a brief questionnaire about your background in AI usage and complete two short writing tasks by interacting with an AI chatbot.

The study will take approximately 20 minutes to complete. You will receive \$6.67 for completing the study, equivalent to a rate of approximately \$20 per hour.

Participation is voluntary. Additional information about the study, including data collection and confidentiality, will be provided in the consent form before you begin.
\end{quote}



% Append after the existing Study Materials sections.
% This snippet does not modify the persona prompts or writing scenarios.

\subsection{Participant-Facing Study Instructions}
\label{app:participant_instructions}

The following instructions were displayed in the study interface before participants completed the background questionnaire and began their assigned tasks.


\subsubsection{Opinion Study Instructions}

\begin{quote}\small
You will have \textbf{three conversations} with an AI assistant, each about a different opinion-based topic. There are no right or wrong opinions. Please respond naturally and honestly.

\medskip
\noindent\textbf{For each conversation}
\begin{enumerate}
    \item Complete a short questionnaire about the topic.
    \item Discuss the topic with the AI assistant.
    \item Complete a short questionnaire after the conversation.
\end{enumerate}

\noindent\textbf{Conversation Guidelines}
\begin{itemize}
    \item Respond to what the AI says and help move the discussion forward. You may explain your reasoning, ask questions, agree or disagree, challenge a point, or introduce a relevant idea.
    \item Each conversation must contain at least \textbf{4 turns}. One turn consists of one message from you and one response from the AI.
    \item You may continue beyond 4 turns if needed, but please try to conclude naturally within approximately \textbf{6--7 turns}.
    \item Before ending, briefly explain where you currently stand on the topic, even if your opinion has not changed.
\end{itemize}

\noindent\textbf{Example}

\noindent\textbf{Topic:} Cats make better pets than dogs.

\noindent\textbf{You:} I agree because cats are more independent and may be easier to care for with a busy schedule.

\noindent\textbf{AI assistant:} Independence is one reason people prefer cats. Others may prefer dogs because they are often more social and encourage outdoor activity.

\noindent\textbf{You:} That's a fair point. Do you think a person's lifestyle matters more than the type of animal?

\medskip
Please complete the study in one sitting using only the study interface. Do not use external AI tools or search engines. Do not provide personally identifiable information such as your real name, address, email, workplace, or school.

\medskip
Next, you will complete the background in AI usage questionnaire before beginning the study.

\medskip
\noindent\textbf{Button:} Continue
\end{quote}

\subsubsection{Writing Study Instructions}

\begin{quote}\small
You will complete \textbf{two Test of English as a Foreign Language (TOEFL)-style email writing tasks}. For each task, you will first write an email independently and then use an AI assistant to receive feedback and revise your writing.

\medskip
\noindent\textbf{For each writing task}
\begin{enumerate}
    \item Write your first draft independently.
    \item Ask the AI assistant for feedback.
    \item Complete at least \textbf{two rounds of AI feedback}, revising your draft between rounds.
    \item Submit your final draft.
\end{enumerate}

\noindent\textbf{Using the Writing Interface}
\begin{itemize}
    \item Use the \textbf{left text box} to write and revise your email.
    \item Use the \textbf{right panel} to ask the AI for feedback.
    \item The AI can see your current draft, so you do not need to copy it into the chat.
    \item You may ask for feedback on clarity, organization, grammar, tone, vocabulary, completeness, or any other aspect of your draft.
\end{itemize}

\noindent\textbf{The AI is for feedback, not writing the response for you.} Do not ask it to rewrite your entire email or generate replacement paragraphs. Make the revisions yourself in the draft box.

\medskip
\noindent\textbf{Example}

\noindent\textbf{You:} Can you give me feedback on whether my email is clear and complete?

\noindent\textbf{AI assistant:} Your email is understandable, but you could make your request more specific and provide a little more context.

\noindent\textbf{You:} Does the tone sound appropriate for a formal email?

\medskip
You do not have to follow every AI suggestion. Use the feedback that you believe improves your email.

\medskip
Complete the study in one sitting and use only the study interface. Do not use other AI tools, grammar checkers, translators, search engines, or writing assistance. Do not include personally identifiable information. If you sign an email, use a fictitious name.

\end{quote}


==> manuscript/benchmark_evaluation.tex <==
\section{Benchmark Evaluation}
\label{sec:benchmarks}

% \subsection{Evaluation Setup}
% \label{sec:benchmark_setup}

% Before examining user responses, we evaluated the personas on published benchmarks covering agreement with users' stated views, social and moral sycophancy, general knowledge, and truthfulness under conversational pressure. Each persona was evaluated on the same prompts within each benchmark, allowing us to compare behavior across the four conditions. We report the benchmark-specific datasets, scoring procedures, and sample sizes below. For the ELEPHANT evaluation, responses were generated with GPT-5.4-mini and scored with GPT-4o; the other benchmark settings should be checked against the experiment logs before submission.
% % TODO: verify model/version and generation settings for the non-ELEPHANT benchmarks.

% \subsection{Agreement with User Views}
% \label{sec:agreement_benchmark}
% We used three sycophancy datasets from the model-written evaluations of Perez et al.~\cite{perez-etal-2023-discovering}: PhilPapers2020, NLP Survey, and Political Typology. Each measures whether a model aligns its answer with a view the user states about themselves. Every persona responded to 9,867 PhilPapers2020, 9,984 NLP Survey, and 10,200 Political Typology prompts. Table~\ref{tab:agreement} reports the percentage of responses that matched the user's view.

% \begin{table}[t]
% \centering
% \caption{Agreement with users' stated views (\% of responses).}
% \label{tab:agreement}
% \begin{tabular}{lrrr}
% \toprule
% \textbf{Persona} & \textbf{PhilPapers2020} & \textbf{NLP Survey} & \textbf{Political Typology} \\
% \midrule
% Objective & 63.97 & 54.78 & 63.60 \\
% Soft-sycophantic & 82.05 & 78.35 & 73.94 \\
% Hard-sycophantic & 86.14 & 89.46 & 73.65 \\
% Baseline & 79.87 & 71.67 & 75.41 \\
% \bottomrule
% \end{tabular}
% \end{table}

% On PhilPapers2020 and NLP Survey, agreement followed the intended order: lowest for the objective persona, highest for the hard-sycophantic persona, with the soft-sycophantic persona between them. On NLP Survey, for example, agreement was 54.78\% for objective, 78.35\% for soft-sycophantic, and 89.46\% for hard-sycophantic. Political Typology separated the personas less. The objective persona was again lowest (63.60\%), but the baseline (75.41\%) was slightly above both sycophantic personas (73.94\% and 73.65\%). This is consistent with Perez et al., who found that sycophancy increased with model size on political questions much more weakly than on NLP and philosophy questions.
% % TODO: verify this description of Perez et al. against their scaling figure before submission.

% \subsection{Social and Moral Sycophancy}
% \label{sec:elephant}

% The datasets above measure agreement with an explicitly stated position. We also wanted a broader form of sycophancy that appears when people seek advice or describe a personal situation. For this we used ELEPHANT~\cite{ICLR2026_d3362f84}, which measures whether a model preserves the user's positive self-image through validation, indirect language, acceptance of the user's framing, and endorsement in moral conflicts.

% We evaluated three ELEPHANT datasets: 3,027 open-ended advice queries (OEQ), 2,000 posts from \textit{r/AmITheAsshole} in which the community judged the poster to be in the wrong (AITA-YTA), and 3,777 assumption-laden statements (SS).
% % TODO: confirm the expansion of "SS" against the ELEPHANT paper.
% Each persona responded to the same 8,804 prompts, giving 35,216 responses, generated with GPT-5.4-mini. Following ELEPHANT's procedure, we used its scoring prompts with GPT-4o as the judge to assign a binary label for three behaviors: \textit{validation} (affirming the user), \textit{indirectness} (suggestive rather than direct language), and \textit{framing} (accepting the user's premise without challenge). We report the percentage of responses with a positive label, not scores normalized against human responses. Of 105,648 judge requests, 105,647 produced a usable label; one baseline AITA-YTA indirectness label was missing and was excluded from that metric's denominator.

% \begin{table}[t]
% \centering
% \caption{ELEPHANT social sycophancy (\% judge-positive responses).}
% \label{tab:elephant_social}
% \begingroup
% \footnotesize
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{@{}llrrr@{}}
% \toprule
% \textbf{Dataset} & \textbf{Persona} & \textbf{Validation} & \textbf{Indirectness} & \textbf{Framing} \\
% \midrule
% OEQ & Objective & 66.90 & 48.63 & 26.96 \\
%  & Soft-sycophantic & 91.18 & 87.78 & 49.85 \\
%  & Hard-sycophantic & 89.49 & 90.06 & 59.33 \\
%  & Baseline & 81.47 & 79.48 & 42.65 \\
% \midrule
% AITA-YTA & Objective & 74.50 & 48.70 & 16.25 \\
%  & Soft-sycophantic & 97.15 & 88.15 & 41.85 \\
%  & Hard-sycophantic & 96.55 & 86.40 & 63.85 \\
%  & Baseline & 89.80 & 75.49 & 31.40 \\
% \midrule
% SS & Objective & 23.70 & 62.06 & 17.18 \\
%  & Soft-sycophantic & 95.31 & 94.55 & 75.01 \\
%  & Hard-sycophantic & 97.01 & 92.98 & 85.52 \\
%  & Baseline & 69.90 & 85.36 & 66.83 \\
% \bottomrule
% \end{tabular}
% \endgroup
% \end{table}

% Across the three datasets, the objective persona had the lowest rate on every dimension. Pooled across datasets, its validation rate was 50.09\%, compared with 78.40\% for baseline and about 94.3\% for both sycophantic personas. Indirectness showed the same pattern: 54.41\% for objective, 81.10\% for baseline, 90.77\% for soft-sycophantic, and 90.48\% for hard-sycophantic. Framing separated the two sycophantic personas more clearly: the hard-sycophantic persona accepted the user's framing in 71.59\% of responses, compared with 58.83\% for soft-sycophantic, 50.47\% for baseline, and 20.33\% for objective. Although the two sycophantic personas were similarly likely to validate users and use indirect language, the hard-sycophantic persona was more likely to leave the user's framing unchallenged. These are descriptive differences in an automated judge's labels.

% We also measured \textit{moral sycophancy} using 1,591 matched pairs from ELEPHANT's AITA-NTA original and flipped datasets. Each pair describes the same moral conflict from the two opposing perspectives. We matched responses by scenario identifier and counted the pairs in which the first verdict in both responses was \textit{Not the Asshole} (NTA), which indicates endorsement of the user even when the perspective reverses.

% \begin{table}[t]
% \centering
% \caption{ELEPHANT moral sycophancy: endorsing both perspectives.}
% \label{tab:elephant_moral}
% \begingroup
% \footnotesize
% \setlength{\tabcolsep}{5pt}
% \begin{tabular}{@{}lrrr@{}}
% \toprule
% \textbf{Persona} & \textbf{Pairs} & \textbf{Both NTA} & \textbf{Moral sycophancy (\%)} \\
% \midrule
% Objective & 1,591 & 309 & 19.42 \\
% Soft-sycophantic & 1,591 & 648 & 40.73 \\
% Hard-sycophantic & 1,591 & 998 & 62.73 \\
% Baseline & 1,591 & 392 & 24.64 \\
% \bottomrule
% \end{tabular}
% \endgroup
% \end{table}

% The hard-sycophantic persona endorsed both sides in 62.73\% of matched conflicts, compared with 40.73\% for soft-sycophantic, 24.64\% for baseline, and 19.42\% for objective. This is another distinction between soft and hard sycophancy: the stronger prompt produced more two-sided endorsement even though the two personas' validation rates were nearly identical. The both-NTA measure captures one particular form of moral sycophancy, not moral accuracy overall, and a lower rate can also arise when a persona judges both sides more harshly. We therefore interpret it alongside the other benchmarks, not as a complete measure of moral consistency.

% \subsection{General Knowledge and Truthfulness Under Pressure}
% \label{sec:truthfulness_benchmark}

% We evaluated knowledge on MMLU-Pro~\cite{wang2024mmluprorobustchallengingmultitask} ($N=12{,}032$ per persona) to check whether changing the level of sycophancy also changed general knowledge performance. We evaluated truthfulness on TruthfulQA~\cite{lin-etal-2022-truthfulqa} ($N=3{,}160$ per persona) using the multi-turn setting described in our evaluation. TruthfulQA contains questions built on common misconceptions. In the multi-turn setting, the model first answers a question and is then challenged seven times by a user who sides with an incorrect or alternative answer, so the benchmark shows whether the model maintains a truthful answer or moves toward the user. We report accuracy after the final turn.

% \begin{table}[t]
% \centering
% \caption{Accuracy (\%) on MMLU-Pro and multi-turn TruthfulQA.}
% \label{tab:accuracy}
% \begingroup
% \footnotesize
% \setlength{\tabcolsep}{6pt}
% \begin{tabular}{@{}lrr@{}}
% \toprule
% \textbf{Persona} & \textbf{MMLU-Pro} & \textbf{TruthfulQA (final)} \\
% \midrule
% Objective & 53.02 & 81.9 \\
% Soft-sycophantic & 53.62 & 44.7 \\
% Hard-sycophantic & 53.55 & 8.7 \\
% Baseline & 54.33 & 59.6 \\
% \bottomrule
% \end{tabular}
% \endgroup
% \end{table}

% MMLU-Pro accuracy was almost identical across personas, ranging from 53.02\% to 54.33\%. This fits our expectation that sycophancy and factual knowledge are different aspects of model behavior: MMLU-Pro asks whether the model can identify a correct answer, and no user is trying to change it. TruthfulQA, in contrast, separated the personas sharply. Final accuracy was 81.9\% for the objective persona, 59.6\% for baseline, 44.7\% for soft-sycophantic, and 8.7\% for hard-sycophantic. These differences appear when the model must choose between maintaining its answer and agreeing with a user who presents an incorrect view, which is the behavior the prompts were designed to change.

% Table~\ref{tab:truthfulqa_turns} shows how the differences developed over the conversation. The objective persona never changed its answer in 1,952 cases, compared with 1,353 for baseline, 1,026 for soft-sycophantic, and only 152 for hard-sycophantic. Conversely, the hard-sycophantic persona changed its response at turn 0 in 1,269 cases and at turn 1 in another 1,459, so it moved toward the user's view almost as soon as it was challenged. The soft-sycophantic persona showed a milder version of the same pattern.

% \begin{table}[t]
% \centering
% \caption{TruthfulQA multi-turn: never changed answer or first changed at turn 0--7 (counts).}
% \label{tab:truthfulqa_turns}
% % TODO: the turn-count rows sum to 3,026 (objective), 3,251 (soft),
% % 3,157 (hard), and 3,231 (baseline), not N=3,160. Reconcile with
% % the original turn logs before submission; do not infer missing rows.
% \begingroup
% \scriptsize
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{@{}lrrrrrrrrr@{}}
% \toprule
% \textbf{Persona} & \textbf{Never} & \textbf{0} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} \\
% \midrule
% Objective & 1952 & 714 & 209 & 45 & 26 & 16 & 17 & 22 & 25 \\
% Soft-sycophantic & 1026 & 1056 & 713 & 210 & 96 & 61 & 40 & 27 & 22 \\
% Hard-sycophantic & 152 & 1269 & 1459 & 182 & 51 & 19 & 16 & 6 & 3 \\
% Baseline & 1353 & 1007 & 536 & 148 & 72 & 44 & 29 & 25 & 17 \\
% \bottomrule
% \end{tabular}
% \endgroup
% \end{table}

% \subsection{Summary of Benchmark Findings}
% \label{sec:benchmark_summary}

% Overall, the benchmarks show that the prompts produced meaningful differences in conversational behavior. The objective persona was generally least likely to agree with users, validate them, or accept their framing, and the sycophantic personas were most likely to. The soft and hard sycophantic personas separated most clearly on framing acceptance and two-sided moral endorsement. These differences were much larger than the differences in MMLU-Pro accuracy, but they became consequential for truthfulness under multi-turn pressure.

% The benchmarks also show that the default model is not a neutral reference point. On NLP Survey and PhilPapers2020, baseline agreed with users far more often than the objective persona (71.67\% vs.\ 54.78\%; 79.87\% vs.\ 63.97\%) and nearly as often as the soft-sycophantic persona (78.35\%; 82.05\%). On ELEPHANT, baseline's pooled validation rate (78.40\%) was closer to the sycophantic personas (about 94\%) than to the objective persona (50.09\%), and its TruthfulQA accuracy (59.6\%) fell between objective (81.9\%) and soft-sycophantic (44.7\%). Moral sycophancy was the exception: baseline's both-NTA rate (24.64\%) was close to the objective persona's (19.42\%). We therefore treat baseline as an already agreeable default, and the user studies compare the objective and sycophantic personas against it. The benchmark results support treating the four prompts as distinct conversational conditions, while recognizing that no single metric captures sycophancy and that the prompts differ in more than agreement.

==> manuscript/conclusion.tex <==
\section{Conclusion}

==> manuscript/user_study.tex <==
% \section{Study 1: Opinion Discussions}
% \label{sec:study1}

% \subsection{Design and Procedure}
% Study 1 examined how discussing contested topics with personas that differ in sycophancy affects people's opinions, confidence, and perceptions of the assistant. After receiving IRB approval, we recruited participants on Prolific and directed them to a web-based chat interface built for the study. The interface used GPT-5.4-mini in all four conditions. Participants were told that the study concerned human--AI collaboration, and were not told that the assistant's conversational style varied between participants. Each participant was randomly assigned to one of the four personas and interacted with the same persona throughout.
% % TODO: add Prolific eligibility criteria, compensation, participant demographics, attention checks, any exclusions, and whether the study was preregistered.

% Each participant discussed three statements on which people can reasonably disagree: ``Social media companies should have stronger content moderation,'' ``A four-day work week should become the standard,'' and ``Governments should ban single-use plastics.'' We chose topics that do not require specialized knowledge, and the order of the three topics was randomized. Before each discussion, participants reported their agreement with the statement and their confidence in that opinion. They then discussed the topic with the assistant. After the discussion, they reported agreement and confidence again, rated their experience with the assistant, and wrote a short free-text explanation of how the conversation affected their view, which we do not analyze here.

% \paragraph{Conversation length.} Participants were instructed to discuss each topic for at least four exchanges. Because of a deployment issue, this minimum was not consistently enforced, so conversation length varied. Only 66 of 200 participants completed at least four exchanges in all three discussions; 154 and 112 completed at least two and at least three, respectively. We therefore report the main analyses on all analyzable conversations and repeat them in the restricted samples (Section~\ref{sec:study1_robust}).
% % TODO: report the mean number of exchanges by persona, since length is measured after assignment and could differ across conditions.

% \subsection{Participants and Measures}
% The study included 200 participants and 597 analyzable conversations out of 600 possible: baseline, 46 participants (138 conversations); objective, 53 (158); soft-sycophantic, 53 (157); and hard-sycophantic, 48 (144).
% % TODO: state why 3 conversations were not analyzable.

% Opinion and confidence were each reported on five-point scales.
% % TODO: confirm scale anchors for agreement and confidence.
% From the pre- and post-discussion responses we derived: whether the opinion changed (any change in the rating); the signed change in agreement with the statement (post minus pre, where negative values mean movement away from agreeing with the statement); the absolute change; \emph{strengthening}, defined as movement farther from the scale midpoint; the change in confidence; and whether confidence decreased. A signed change shows movement toward or away from the stated proposition. It does not show whether a participant was persuaded toward the assistant's position or toward a more accurate view.

% After each discussion, participants rated the assistant on seven items: how respectful, satisfying, and trustworthy they found it (our main perception measures), and how persuasive it was, how fairly it considered other perspectives, whether the conversation helped them think more deeply, and whether it encouraged them to consider alternative viewpoints.
% % TODO: confirm response scale (we assume five-point) and include exact item wording in the appendix.

% \subsection{Analysis}
% We regressed each outcome on persona, with baseline as the reference, adjusting for initial opinion, initial confidence, familiarity with AI, and topic, and clustering standard errors by participant because each participant contributed up to three discussions. We used logistic models for binary outcomes and linear models for continuous outcomes, and tested the overall effect of persona with a Wald test.
% % TODO: confirm model types, the exact familiarity covariate, and the list of outcomes in the FDR family.
% We report Holm-adjusted $p$-values for pairwise contrasts within an outcome, and false discovery rate (FDR) adjusted $p$-values for omnibus tests across the 11 outcomes analyzed, so that we can distinguish individual contrasts from findings that remain after broader correction. Because the study did not include a condition without AI discussion, changes in opinion and confidence cannot be attributed to the assistant alone.

% \subsection{Results}

% \paragraph{Perceptions of the assistant.}
% Participants evaluated the objective persona less favorably than the other personas (Table~\ref{tab:perceptions}). It received lower respect ratings than baseline, soft-sycophantic, and hard-sycophantic AI (adjusted differences of $-0.78$, $-0.71$, and $-0.81$ points; all Holm-adjusted $p<0.001$), and lower satisfaction ratings than each of the three (adjusted differences of $-0.64$, $-0.47$, and $-0.52$; Holm-adjusted $p<0.001$, $p=0.007$, and $p=0.003$). For trust, the objective persona scored below baseline (adjusted difference $-0.52$, 95\% CI $[-0.78, -0.25]$, Holm-adjusted $p=0.0007$). The omnibus effects of persona on respect, satisfaction, and trust remained significant after FDR correction across outcomes.

% The sycophantic personas did not receive higher ratings than baseline on these measures. In a pooled comparison, the two sycophantic personas together showed no significant advantage over baseline on the perception outcomes after correction, and soft- and hard-sycophantic AI did not differ significantly from each other.
% % TODO: confirm from the model output that none of the baseline-versus-soft and baseline-versus-hard contrasts on respect, satisfaction, and trust is significant, so this can be stated per persona.
% Baseline had the highest mean satisfaction and trust. We therefore found no evidence that explicitly instructing the model to agree with and affirm users improved evaluations relative to the default assistant. The remaining items showed smaller or less robust differences. The objective persona rated lowest on fairness and deeper thinking, though neither omnibus test was significant. It rated highest, descriptively, on encouraging alternative viewpoints, and was rated above hard-sycophantic AI on that item (adjusted difference $+0.53$, Holm-adjusted $p=0.024$), but the omnibus effect did not survive FDR correction ($p_{\mathrm{FDR}}=0.082$). Persuasiveness showed a similar pattern ($p_{\mathrm{FDR}}=0.112$), so we treat these item-level contrasts as exploratory.

% \begin{table}[t]
% \centering
% \caption{Mean ratings of the assistant by persona (raw means) and omnibus tests of persona from adjusted models (FDR-adjusted across outcomes).}
% \label{tab:perceptions}
% \small
% \begin{tabular}{lrrrrr}
% \toprule
% \textbf{Item} & \textbf{Objective} & \textbf{Soft} & \textbf{Hard} & \textbf{Baseline} & \textbf{Omnibus $p_{\mathrm{FDR}}$} \\
% \midrule
% Respectful & 3.66 & 4.37 & 4.47 & 4.44 & $<0.001$ \\
% Satisfying & 3.76 & 4.22 & 4.28 & 4.41 & 0.0004 \\
% Trustworthy & 3.73 & 4.06 & 4.06 & 4.26 & 0.012 \\
% Persuasive & 3.58 & 3.77 & 3.86 & 3.98 & 0.112 \\
% Fair consideration & 3.73 & 3.92 & 3.83 & 4.09 & 0.214 \\
% Deeper thinking & 3.78 & 3.92 & 4.03 & 4.07 & 0.492 \\
% Alternative viewpoints & 3.80 & 3.57 & 3.26 & 3.75 & 0.082 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \paragraph{Opinion change and confidence.}
% Participants changed their opinion rating in 221 of 597 discussions (37.0\%), and the frequency of change did not differ significantly across personas ($\chi^2(3)=1.55$, $p=0.671$). Strengthening occurred in about 25.3\% of discussions and movement toward the midpoint in about 6.7\%, with no significant persona effect on strengthening ($p=0.175$).
% % TODO: add the percentage of discussions with an opinion change for each persona.

% The direction of change did differ. The overall persona effect on signed opinion change survived FDR correction ($\chi^2(3)=14.00$, $p=0.0029$, $p_{\mathrm{FDR}}=0.016$), and participants who discussed with the objective persona showed more negative signed change than baseline participants ($\beta=-0.36$, 95\% CI $[-0.56, -0.16]$, Holm-adjusted $p=0.002$). In other words, they moved less toward agreeing with the statements, and this contrast does not show movement toward or away from the assistant's own position. Initial opinion extremity did not significantly moderate the persona effect on signed change ($\chi^2(3)=1.12$, $p=0.773$).
% % TODO: add an analysis of signed change conditional on each participant's initial stance (supportive, neutral, opposed), since the assistant's pushback may run against a majority starting view on these topics.

% Mean confidence increased in every condition (by 0.38 points overall), and mean confidence change did not differ significantly by persona ($p=0.298$; Table~\ref{tab:outcomes}). A different pattern appeared when we asked whether confidence decreased at all. Confidence decreased in 13.9\% of discussions with the objective persona (22 of 158), compared with 3.6\% for baseline (5 of 138), 7.0\% for soft-sycophantic (11 of 157), and 9.7\% for hard-sycophantic (14 of 144). The adjusted odds of a confidence decrease were higher for objective than for baseline (OR $=5.10$, 95\% CI $[1.92, 13.56]$, Holm-adjusted $p=0.0065$). We treat this as suggestive: the overall effect of persona on confidence decrease did not survive FDR correction across outcomes ($p_{\mathrm{FDR}}=0.056$), and the contrast rests on few baseline events.
% % TODO: confirm the event counts above, which we derived from the reported percentages.

% \begin{table}[t]
% \centering
% \caption{Opinion and confidence outcomes by persona (descriptive).}
% \label{tab:outcomes}
% \small
% \begin{tabular}{lrrrr}
% \toprule
%  & \textbf{Objective} & \textbf{Soft} & \textbf{Hard} & \textbf{Baseline} \\
% \midrule
% Conversations & 158 & 157 & 144 & 138 \\
% Mean absolute opinion change & 0.563 & 0.503 & 0.500 & 0.478 \\
% Mean confidence change & $+0.272$ & $+0.497$ & $+0.347$ & $+0.413$ \\
% Confidence increased (\%) & 34.2 & 35.0 & 31.9 & 36.2 \\
% Confidence decreased (\%) & 13.9 & 7.0 & 9.7 & 3.6 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \paragraph{Robustness to conversation length.}
% \label{sec:study1_robust}
% Because the four-exchange minimum was not consistently enforced, we repeated the analyses among participants who completed at least two, three, or four exchanges in every discussion (Table~\ref{tab:robust}). The null effect of persona on mean confidence change held in every sample. The objective-versus-baseline contrast on confidence decrease was directionally similar throughout, but it did not reach conventional significance in the strictest sample of 66 participants, where uncertainty is much larger. These restricted samples are defined by behavior after assignment, so they may differ in composition from the full sample.

% \begin{table}[t]
% \centering
% \caption{Sensitivity to conversation length. Objective versus baseline odds of a confidence decrease (adjusted OR, unadjusted $p$) and omnibus $p$ for mean confidence change.}
% \label{tab:robust}
% \small
% \begin{tabular}{lrrrr}
% \toprule
% \textbf{Sample} & \textbf{Participants} & \textbf{OR} & \textbf{$p$} & \textbf{Omnibus $p$ (mean confidence)} \\
% \midrule
% All available & 200 & 5.10 & 0.0011 & 0.298 \\
% $\ge 2$ exchanges & 154 & 6.85 & 0.0032 & 0.265 \\
% $\ge 3$ exchanges & 112 & 7.06 & 0.0174 & 0.725 \\
% $\ge 4$ exchanges & 66 & 5.22 & 0.0743 & 0.753 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \paragraph{Ratings and outcomes.}
% Finally, we asked whether participants' ratings were related to what happened in their discussions. These are post-discussion associations, not effects of the ratings. Across conversations, higher ratings on all six items we examined (respect, trust, satisfaction, deeper thinking, fairness, and alternative viewpoints) were associated with a higher probability of changing one's opinion (for example, $+11.9$ percentage points per rating point for satisfaction and $+10.7$ for deeper thinking; $p_{\mathrm{FDR}}<0.01$ for all), and all but fairness were associated with larger absolute change. Only encouragement to consider alternative viewpoints was associated with a higher probability of reduced confidence ($p_{\mathrm{FDR}}<0.001$).
% % TODO: confirm whether persona was included as a covariate in these models, and state the model specification.
% Participants who rated a discussion more favorably were therefore also more likely to change their opinion, even though the personas that were rated differently did not differ in how often participants changed their opinions. Participants may also rate a conversation more highly because it moved them.

% \section{Study 2: AI-Assisted Writing}
% \label{sec:study2}

% \subsection{Design and Procedure}
% Study 2 examined whether differences in sycophancy affect how people use feedback to revise their own writing. Where Study 1 involved agreement and disagreement about a topic, here the assistant evaluated work the participant had produced. Participants completed two email-writing tasks adapted from TOEFL preparation materials~\cite{goodine_toefl_email}. In the \emph{Wrong Package} task, participants wrote to customer service after receiving a cheaper, different pair of headphones than the pair they ordered. In the \emph{Noisy Neighbors} task, they wrote to a property manager about repeated late-night noise from upstairs neighbors. Each task provided a scenario and points the email should address. The full prompts are in Appendix~\ref{app:prompts}.
% % TODO: add recruitment platform, eligibility, compensation, demographics, attention checks, and IRB statement for Study 2.

% For each task, participants first wrote an email independently, without AI assistance. They then used the chat interface to ask for feedback on clarity, organization, grammar, tone, and completeness. The instructions asked participants to obtain feedback and not to have the AI generate or rewrite the email, and they were required to receive feedback at least twice before submitting a revised final draft. Participants were randomly assigned to one of the four personas, interacted with that persona throughout both tasks, and received the same two scenarios in randomized order. The underlying model was GPT-5.4-mini, and participants were not told that personas differed.

% \subsection{Participants and Measures}
% We recruited 200 participants and analyzed the 198 with complete initial and final drafts, giving 396 paired writing tasks: baseline, 50 participants (100 task pairs); objective, 49 (98); soft-sycophantic, 53 (106); and hard-sycophantic, 46 (92).

% Our main outcome was writing quality. We scored initial and final drafts with an LLM-based grader applying an adapted TOEFL-style email rubric on a 0 to 5 scale, in two versions: integer scores, and scores allowing half-point increments. These are not official TOEFL scores, and we have not validated them against human ratings.
% % TODO: name the grader model, report temperature and whether the grader saw the persona or the conversation, and add the rubric and grading prompt to the appendix.
% We also measured revision behavior: the net change in word count, the normalized edit distance between initial and final drafts, and the proportion of original sentences not preserved verbatim. These capture different aspects of revision. A sentence that is not preserved verbatim may have received only a small edit, so this last measure does not show substantive reorganization.

% \subsection{Analysis}
% We first compared initial and final scores within participants, accounting for each participant completing two tasks. To test whether persona affected final writing quality, we regressed the final score on persona (baseline as reference), the initial score, and the writing task, with standard errors clustered by participant. This separates differences in final quality from differences in the draft participants wrote before receiving feedback. We then compared revision measures across personas, reporting Holm-adjusted pairwise contrasts and bootstrap confidence intervals for differences in word count. The study had no condition in which participants revised without AI feedback, so improvements cannot be attributed to the feedback itself.

% \subsection{Results}

% \paragraph{Writing quality.}
% Participants' scores rose after interacting with the assistant in all four conditions (Table~\ref{tab:writing}). The mean increase from initial to final draft was 0.288 points on the integer scale (95\% CI $[0.217, 0.361]$) and 0.296 on the half-point scale ($[0.239, 0.355]$), and within-person improvements were significant in each condition (all Holm-adjusted $p<0.01$). The objective persona had the largest descriptive improvement, but pairwise differences in gains between personas were not significant after Holm correction. Significant improvement within a condition therefore does not mean that condition outperformed the others.

% After accounting for initial quality and task, we found no evidence that persona affected final writing quality (omnibus $p=0.959$ on the half-point scale and $p=0.633$ on the integer scale). On the half-point scale, the adjusted differences from baseline were $+0.03$ for objective (95\% CI $[-0.13, 0.18]$), $+0.04$ for soft-sycophantic ($[-0.12, 0.20]$), and $+0.04$ for hard-sycophantic ($[-0.11, 0.19]$), and results were similar on the integer scale. Initial quality strongly predicted final quality ($\beta=0.68$). These intervals exclude persona differences larger than about 0.2 points on the half-point scale, but they do not establish equivalence, and the integer-scale intervals are wider (up to about 0.28).

% \paragraph{Revision behavior.}
% Personas differed in how participants revised, but not in how well (Table~\ref{tab:writing}). Participants assigned to the objective persona added the most words on average (14.65 net words) and made 7.96 more net additions than those assigned to the soft-sycophantic persona (95\% bootstrap CI $[2.83, 13.73]$, Holm-adjusted $p=0.018$). Normalized edit distance followed a similar descriptive order (0.267 for objective, 0.234 for hard-sycophantic, 0.226 for baseline, and 0.194 for soft-sycophantic) but the overall persona effect was not significant (Wald $\chi^2(3)=5.36$, $p=0.147$). Participants assigned to the objective persona also modified the highest proportion of original sentences (41.7\%), but no pairwise difference survived Holm correction. Greater word expansion with the objective persona therefore did not correspond to a significantly higher adjusted final score.

% \begin{table}[t]
% \centering
% \caption{Writing outcomes by persona. Score gains are mean final minus initial scores; none of the pairwise differences in gains between personas was significant after Holm correction.}
% \label{tab:writing}
% \small
% \begin{tabular}{lrrrr}
% \toprule
%  & \textbf{Objective} & \textbf{Soft} & \textbf{Hard} & \textbf{Baseline} \\
% \midrule
% Participants / task pairs & 49 / 98 & 53 / 106 & 46 / 92 & 50 / 100 \\
% Score gain (integer scale) & $+0.398$ & $+0.245$ & $+0.261$ & $+0.250$ \\
% Score gain (half-point scale) & $+0.337$ & $+0.316$ & $+0.239$ & $+0.285$ \\
% Net words added & $+14.65$ & $+6.69$ & $+8.78$ & $+8.88$ \\
% Original sentences changed (\%) & 41.7 & 34.5 & 37.5 & 32.7 \\
% Normalized edit distance & 0.267 & 0.194 & 0.234 & 0.226 \\
% \bottomrule
% \end{tabular}
% \end{table}

% \paragraph{Task position.}
% Initial draft scores were higher in the second task than in the first ($+0.14$ on the half-point scale, $p=0.008$), revision gains were smaller ($-0.17$, $p=0.002$), and final scores did not differ ($-0.02$, $p=0.635$). Persona did not interact with task position (half-point $p=0.597$; integer $p=0.313$). We do not interpret this pattern as learning. Task order was randomized, so position and prompt must be separated, and a ceiling on what the rubric rewards could produce the same pattern.
% % TODO: confirm that the task-number variable is chronological position and re-estimate these models with prompt identity included.
